Kepler: Robust Learning for Faster Parametric Query Optimization

Most existing parametric query optimization (PQO) techniques rely on traditional query optimizer cost models, which are often inaccurate and result in suboptimal query performance. We propose Kepler, an end-to-end learning-based approach to PQO that demonstrates significant speedups in query latency over a traditional query optimizer. Central to our method is Row Count Evolution (RCE), a novel plan generation algorithm based on perturbations in the sub-plan cardinality space. While previous approaches require accurate cost models, we bypass this requirement by evaluating candidate plans via actual execution data and training an ML model to predict the fastest plan given parameter binding values. Our models leverage recent advances in neural network uncertainty in order to robustly predict faster plans while avoiding regressions in query performance. Experimentally, we show that Kepler achieves significant improvements in query runtime on multiple datasets on PostgreSQL.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> coverletter.tex <==
\thispagestyle{empty}
\setcounter{figure}{-1}
\setcounter{table}{-1}
We thank the area chair and reviewers for their valuable comments.  We have incorporated the comments, with paper revisions \textcolor{blue}{highlighted}.

% In Sections A and B, we respond to the meta reviewer comments and individual reviewer comments. 

\vspace{0.15in}
\noindent\textbf{A. Required Changes (Response to Meta Reviewer Comments)}

\begin{enumerate}
%1
\item We moved the RCE experiments. We had them in Section~\ref{subsec:row count evolution} to provide some empirical justification/motivation for RCE, and agree moving them to Section~\ref{sec:experiments} works better.
We also moved the description of candidate plan generation baselines to Section~\ref{sec:related}.

%2
\item We have rewritten most of the experimental evaluation in Section~\ref{sec:experiments}. We reorganized it to present the main results in Section~\ref{subsec:exp_e2e}, followed by supporting evidence of the two main components in Sections~\ref{subsec:analyze_rce} and \ref{subsec:model_exp}. We emphasized the main objectives for our system, and clearly reference them throughout the section. We added emphasis for our key takeaways and metrics as well as more flow content to link the subsection's story together. We also added new experiments and/or new data to improve the tables, including Table~\ref{tab:e2e_stack}, Table~\ref{tab:stack_depth}, and Figure~\ref{fig:ood}. 
%3
\item We reviewed and removed unrigorous experiments. In the specific case of the Bao experiments, we enlisted the help of Ryan Marcus (first author of Bao) in running the Bao experiments to ensure we had fair comparisons. The results are more reasonable, and we have a more concrete/supported explanation for the suboptimality of Bao.  See "Bao on parameterized queries" and Table~\ref{tab:bao} in Section~\ref{subsec:exp_e2e}.
%4
\item We took care to emphasize all experiments that ablate aspects of our method. For RCE, the comparisons against baselines serve to ablate the contribution of RCE. Although our ML method is simple, we show ablation studies on two key aspects: Figure~\ref{fig:stack_model_speedups} ablates the use of SNGP, and Figure~\ref{fig:vocabulary} ablates the use of our max-marginal improvement vocabulary selection.
%5
\item See Changing environments and workloads in Section~\ref{ss:system-overview} and Section~\ref{sec:future_work}.

%6
\item See Changing environments and workloads in Section~\ref{ss:system-overview} and Section~\ref{sec:future_work}.

\item Regarding RCE: Section~\ref{subsec:analyze_rce} now states we intend the justification to be empirical, with content adjusted in "Can RCE discover optimal plans?". The other empirical supporting sections moved to Section~\ref{subsec:analyze_rce} too: "Exponential row count perturbation range", "Query clusters facilitate RCE".
Regarding needing all executions times: Added content to Section~\ref{subsec:training_objectives}. 

\item We agree that this is a very promising future work direction for RCE. In Section~\ref{sec:future_work}, we mentioned that using a generative cardinality estimation model could be used in a similar way to improve RCE.

\item We intended the dataset to be used for algorithmic/modeling research, and added Section~\ref{subsec:dataset_contribution} to state this more clearly.

%10
\item 
\begin{enumerate}
    \item Added new out-of-distribution experiments under "SNGP out-of-distribution detection" in Section~\ref{subsec:model_exp}. See Figure~\ref{fig:ood}. Section~\ref{sec:future_work} mentions incorporating cardinality estimates, which may also help here.
    \item In this table (now Table~\ref{tab:rce_vs_exact}), the RCE average query latency is much faster than the average exact cardinality query latency - a fairly surprising result!
\end{enumerate}

%11
\item We use the same hyperparameters (RCE and model) for all queries (stated in Section~\ref{subsec:setup}). We added a new hyperparameter experiment in "Number of generations $G$" with Table~\ref{tab:stack_depth}. The candidate plan set size is an output of plan cover pruning and we plot the sizes we observed in Figure~\ref{fig:stack_plan_cover_sizes_histogram}. 

%12
\item RCE is better than exact cardinality plans because the latter still suffers from imperfect cost models. We added this explanation to "Can RCE discover optimal plans?" in Section~\ref{subsec:analyze_rce}. The table is now Table~\ref{tab:rce_vs_exact}, and we removed Figure 3 because it was redundant.

\item We overhauled our presentation of RCE, adding an explicit example (Figure~\ref{fig:rce_example}), simplifying the pseudocode in Algorithm~\ref{alg:rce}, and adding a RCE hyperparameters table (Table~\ref{tab:term}).

\end{enumerate}

\vspace{0.15in}
\noindent\textbf{B. Optional Changes (Responses to Individual Reviewers Comments)}

We add more content when a comment was not included in the metareview.

\textbf{Reviewer 1 and 4.}
R1 O2, R4 D3: We have stated more clearly how we picked those queries. We wanted a relatively diverse set of query templates in the overall workload and did not cherry-pick them after running experiments. When we used a subset, we were constrained by computational reasons. We now mention this in Section~\ref{subsec:analyze_rce}'s "Comparison against baselines" and "Can RCE discover optimal plans?".

\textbf{Reviewer 1.}

In addition to the rewrite, we improved the figure placement and double checked figure references.

Thanks for identifying the typos. We've fixed them.

\textbf{Reviewer 2.} 

D2: We added "Training data collection cost" at the end of Section~\ref{subsec:exp_e2e}, which in turn list additional references on the topic: end of Section~\ref{subsec:model_exp}, Section~\ref{subsec:dataset_contribution}, and Section~\ref{sec:future_work}.

\textbf{Reviewer 4.}

O1. Half this comment is addressed in the metareview. We also added content on the approximate approach in Section~\ref{subsec:analyze_rce}'s "Can RCE discover optimal plans?".

D1. We've improved the caption for Figure~\ref{fig:pred_vs_actual_q12_2}. The points are actual vs estimated cardinality of subqueries from query instances of Stack template q12\_2. A perfect estimator would lie on the dashed y=x line.
  
D2. Models are <1 mb each with fast inference times (See Section~\ref{subsec:exp_e2e}).
    
D4. We improved our exposition of clusters in Section~\ref{subsec:analyze_rce}. RCE-all is fastest since RCE-cluster and RCE-instance use subsets of RCE-all plans.



\thispagestyle{empty}
\newpage
\setcounter{page}{1}

% \renewcommand\thefigure{\thesection.\arabic{figure}}    https://braintex.goog/project/6232709040d80900a141a43a
\setcounter{figure}{0}
\setcounter{table}{0}

==> sections/Deprecated__problem_setting.tex <==
DEPRECATED!!!!!!

\section{Problem Setting}
We consider parameterized queries that are repeatedly invoked with different parameter bindings. In a production setting, this may vary from 100s and 1,000,000s times a day. Such queries are specified by a template $Q$ with $m$ parameterized predicates $x_0,...,x_m-1$ of varying data types. We consider a decoupled approach as in \citet{vaidya2021leveraging}: 1. generating a set of $k$ plans $p$, and 2. map $[x_0,...,x_m-1] \mapsto p \in \{p_0,...,p_{k-1}\}$ to achieve lower latency across a workload (mean, tail) than the database’s optimizer. 

% We propose classifying query workloads as containing a combination of (1) templates executed repeatedly with varying parameter bindings and (2) ad-hoc queries. Within each group, the best plan for a query may or may not be sensitive to the bind parameter values. In this work, we focus on repeating, parameter-sensitive queries and treat repeating, non-parameter sensitive queries as a simpler case that can be addressed by our framework. 

% We posit that repeatedly executed query templates are common in a production setting where an application may be issuing queries with parameters bound according to the current user or application request. When such a query is executed 100s to 1,000,000s times a day, spending effort to find an optimal query plan can yield high returns.

% We frame the problem as a classification problem to identify the optimal or near-optimal plan from a set of plans on a per-query basis. This allows us to make the following claims that reflect an emphasis on practical deployment in a production setting: 

% \begin{enumerate}
%     \item Focus on latency priorities: We craft our training objectives to prioritize minimizing empirical tail latencies. The classification framing enables us to avoid the harder problem of generically and accurately predicting execution latency. We only need to identify the optimal plan; we don't need to know precisely how bad the alternatives are. In the scheme of a workload, we additionally posit that we only need to identify a near-optimal plan while we prioritize eliminating tail latencies and avoiding bad plan choices. 
%     \item Focused models and isolation: We propose training models on a per-query template basis. This allows the user to focus ML-interaction only on challenging queries and provides isolation between models to eliminate the risk of wide-spread regressions. 
%     \item Focus on regressions: We prioritize avoiding regressions compared to the status quo. The database optimizer itself is the status quo expert and we defer to it when we cannot confidently make a prediction about the optimal plan choice to avoid unfortunate "guesses" from any ML approach.
%     \item Pay something to get something: In a repeated setting, we can justify investment in identifying both strong plans and an effective parameter binding to plan mapping function. Just as building an index incurs a cost to bring significant gains, Kepler too incurs a training cost to bring significant workload gains.
%     \item Focus on nullifying complex system dynamics: Real world systems have layers of complexity and are difficult to model accurately. Features may be added. Deployment and storage architectures may evolve. Data volumes will grow. By treating the end-to-end system as a black box and periodically re-collecting training data, Kepler automatically adapts to the changing world without explicitly system model actions required by the database developers. 
% \end{enumerate}

This approach has several key advantages in the parameter query optimization setting:

\begin{enumerate}
    \item \textbf{Per-template models.} We train a model per query template, providing isolation from regressions between queries as models iterate over time. 
    \item \textbf{Robustness.} 
    \item \textbf{Training data collection cost.} In a repeated setting, investment in identifying both strong plans and an effective parameter binding to plan mapping function provides continuous benefits to the workload. The Kepler trade-off parallels how building an index incurs a cost to bring significant gains.
    \item Focus on nullifying complex system dynamics: Real world systems have layers of complexity that are difficult to model accurately. Features may be added. Deployment and storage architectures may evolve. Data volumes grow. By treating the end-to-end system as a black box and periodically re-collecting training data, Kepler automatically adapts to the changing world without requiring database developers to explicitly update cost models. 
\end{enumerate}

\subsection{Kepler Value Proposition}

Kepler leverages the expertise of the database query optimizer to generate plan candidates and applies further refinement. Row Count Evolution \ref{subsec:row count evolution} Specifically, 
Kepler creates a search space of query plans by using the query optimizer's suggestions to given queries with varying parameters.
Kepler learns the decision boundaries in the parameter value space to choose the fastest plan for the job, closing the loop with empirical experience instead of relying only on open-loop cost-model estimates. Kepler caters decision boundaries for plan choice to the data and application’s exhibited interaction instead of relying on developer knowledge.

\subsubsection{Kepler Improves Query Performance Manageability}

When the database optimizer's plan selection is suboptimal, a user may apply their query debugging expertise to run experiments and identify a set of hints to force optimizer plan decisions towards the better plan. This process ideally requires:
\begin{enumerate}
    \item Identifying the query as suboptimal
    \item Query bindings that reproduce the issue
    \item A query debugging expert
    \item A method to ensure the new version of the query doesn't cause a different regression
\end{enumerate}

Even when all of the above can be satisfied, the process is not likely repeated periodically to identify new suboptimal queries or ensure that the fixes made previously are still providing benefits. After a version upgrade, data distribution shift, or workload change, the hinted query may now be suboptimal.

Furthermore, if the query is parameter-sensitive and the database optimizer is producing suboptimal plans, \emph{there is no single set of hints} the user can unilaterally provided to avoid regressions somewhere.

\emph{An automated Kepler system can take over all of the above and periodically run checks to determine if any updates are required to prior decisions regarding query plan hints.}

\subsubsection{Kepler Improves Database Development Velocity and Plan Stability}

A database deployment is a shifting landscape of performance characteristics. As features and bugs come and go, Kepler adapts its plan choices automatically to find the headroom wherever it exists. For a given plan-selection short-coming, it may be possible to root-cause the bug and fix it. This process still takes time and does not scale easily as the number of issues that requires a few weeks or months to root-cause, fix and release grows. Kepler can mold plan selection around these bugs by executing training data collection queries, reducing or even eliminating the urgency to fix them in some cases. 

Optimizer upgrades may also change decision boundaries between plan options, which inevitably both positively and adversely affect execution times for a specific query to create a “new normal”. Here too, Kepler will (re)learn the actual new decision boundary to provide the fastest performance amongst the plan options, providing protection against unanticipated and potentially user-specific regressions and consequent fallout.

\subsubsection{Parameter Sensitivity in Production}

Kepler employs empirical observations as a cornerstone of its approach in training an ML model for query plan selection. This contrasts with competing production features such as Oracle Adaptive Cursor, Aurora Managed Plans, and SQL Server Parameter Sniffing, which all lean on their cost models and cardinality estimates when trying to overcome query planning challenges in an adaptive fashion. In all cases, final decision making involves traditional statistics and heuristics. The approaches do not incorporate trained machine learning models.

\begin{enumerate}
    \item Oracle Adaptive Cursor uses selectivity estimates to identify likely similar plans 
    \item Aurora Managed Plans uses its cost model output to compare amongst a fixed set of plan options
    \item SQL Server sniffs parameter bindings and caches a plan for reuse
\end{enumerate}
    
Instead of adjusting greedily as query bind parameters are encountered that do not fit the current mold, Kepler takes a broader view of modeling the bind parameter space to make holistic query plan selection recommendations.

\subsection{Fundamental Limitations}

We would like to make clear some fundamental limitations and non-goals of Kepler:
\begin{enumerate}
    \item We do not support plan predictions for ad-hoc queries at this time
    \item If a query is only lightly repeating, the cost-benefit of Kepler may not be worthwhile \emph{unless} that query's latency is of very high value to the user.
    \item Our current training data collection requirements are unlikely to suit a parameter-sensitive long-running query. Kepler may still make sense as a tool if there's a single optimal plan to identify and occasionally re-verify.
    \item The version presented here has not been evaluated for the effect of changing workloads without re-training. We believe we can extend to this case and consider it to be future work.
    \item The version presented here has not been evaluated with user-defined functions within queries. We believe we can handle this case due to the blackbox end-to-end latency training and we need to run experiments accordingly. 
\end{enumerate}

